Interference and Need Aware Workload Colocation in Hyperscale Datacenters

Datacenters suffer from resource utilization inefficiencies due to the conflicting goals of service owners and platform providers. Service owners intending to maintain Service Level Objectives (SLO) for themselves typically request a conservative amount of resources. Platform providers want to increase operational efficiency to reduce capital and operating costs. Achieving both operational efficiency and SLO for individual services at the same time is challenging due to the diversity in service workload characteristics, resource usage patterns that are dependent on input load, heterogeneity in platform, memory, I/O, and network architecture, and resource bundling. This paper presents a tunable approach to resource allocation that accounts for both dynamic service resource needs and platform heterogeneity. In addition, an online K-Means-based service classification method is used in conjunction with an offline sensitivity component. Our tunable approach allows trading resource utilization efficiency for absolute SLO guarantees based on the service owners' sensitivity to its SLO. We evaluate our tunable resource allocator at scale in a private cloud environment with mostly latency-critical workloads. When tuning for operational efficiency, we demonstrate up to ~50% reduction in required machines; ~40% reduction in Total-Cost-of-Ownership (TCO); and ~60% reduction in CPU and memory fragmentation, but at the cost of increasing the number of tasks experiencing degradation of SLO by up to ~25% compared to the baseline. When tuning for SLO, by introducing interference-aware colocation, we can tune the solver to reduce tasks experiencing degradation of SLO by up to ~22% compared to the baseline, but at an additional cost of ~30% in terms of the number of hosts. We highlight this trade-off between TCO and SLO violations, and offer tuning based on the requirements of the platform owners.

==> COP_algo.tex <==



\textcolor{blue}{One such constraint of the solver is to minimize the number of hosts utilized and the resource fragmentation, such that each job is mapped to exactly one host and job resource requirements are met. Equation~\ref{Goals} shows the primary goal for convergence, as the number of hosts, jobs, and resource counts (like the number of cores, memory capacity) can't be fractions, the constrained optimization problem is solved using Integer Linear Programming by a greedy approach to converge to a result as quickly as possible. Secondary goals include reducing SLI violations and TCO. Other than that, there are other weighted goals added in the packer-solver. A pseudo-code of the vanilla version of the algorithm has been provided in Algorithm~\ref{alg:packer_solver}. There are added constraints for fault-tolerance and redundancy, like the availability of a minimum number of tasks for a particular service to deal with sudden traffic spikes and copies of tasks across geographical regions of datacenters to deal with unforeseen failures. These constraints, along with some others, haven't been depicted in the basic algorithm.}
\\
\textcolor{blue}{
\begin{equation}
\resizebox{\hsize}{!}{
\begin{split}
\label{Goals}
h \in (Hosts Occupied \cup Hosts Free)\\
Minimize(Hosts Occupied)\\
k \in [CPU, MEMORY]\\
h_{\textbf{limit}}(k) = host\hspace{0.1cm}resource \hspace{0.1cm}capacity\hspace{0.1cm} for\hspace{0.1cm}  resource\hspace{0.1cm}k\\
t_{\textbf{limit}}(k) = task\hspace{0.1cm}resource \hspace{0.1cm}requirement\hspace{0.1cm} for\hspace{0.1cm} resource\hspace{0.1cm}k\\
h_{\textbf{tasks}}= tasks\hspace{0.1cm} assigned\hspace{0.1cm} to\hspace{0.1cm} host\hspace{0.1cm} h\\
Fragmentation(k) = \sum_{\substack{\tiny \forall h\in Hosts Occupied}}(h_{\textbf{limit}}(k) - (\sum_{\substack{\forall t \in h_{\textbf{tasks}}}}(t_{\textbf{limit}}(k)))  )
\end{split}
}
\end{equation}
}


\begin{algorithm}
\textcolor{blue}{
$Hosts=(Hosts Occupied \cup Hosts Free)$\\
%$J=(Jobs)$\\
%$RR=(Per\hspace{0.1cm}Task\hspace{0.1cm}Resource\hspace{0.1cm}Requirements\hspace{0.1cm}for\hspace{0.1cm}[CPU, MEMORY])$\\
$k \in [CPU, MEMORY] $\\
$l \in [CPU, Memory\hspace{0.1cm}Bandwidth, Network\hspace{0.1cm}Bandwidth] \\
%$SS=(Per\hspace{0.1cm}Task\hspace{0.1cm}Sensitivity\hspace{0.1cm}Scores\hspace{0.1cm}for\\ \hspace{0.1cm}[CPU, Memory\hspace{0.1cm}Bandwidth, Network\hspace{0.1cm}Bandwidth])$
%$RD=Resource\hspace{0.1cm}Dimensions\hspace{0.1cm}(CPU, Memory)$\\
%$SD=Sensitivity\hspace{0.1cm}Dimensions\hspace{0.1cm}\\(CPU, Memory\hspace{0.1cm}Bandwidth, Network\hspace{0.1cm}Bandwidth)$\\
$h_{\textbf{limit}}(k) = host\hspace{0.1cm}resource \hspace{0.1cm}capacity\hspace{0.1cm} for\hspace{0.1cm}  resource\hspace{0.1cm}k$\\
$t_{\textbf{limit}}(k) = task\hspace{0.1cm}resource \hspace{0.1cm}requirement\hspace{0.1cm} for\hspace{0.1cm} resource\hspace{0.1cm}k$\\
$t_{\textbf{sensitivity}}(l) = task\hspace{0.1cm}sensitivity \hspace{0.1cm}score\hspace{0.1cm} for\hspace{0.1cm} l\hspace{0.1cm}on\hspace{0.1cm}base\hspace{0.1cm}architecture$\\
$t_{\textbf{norm}}(l) = task\hspace{0.1cm}sensitivity \hspace{0.1cm}score\hspace{0.1cm} for\hspace{0.1cm} l\hspace{0.1cm}on\hspace{0.1cm}h_{\textbf{arch}}$\\
$h_{\textbf{tasks}}= tasks\hspace{0.1cm} assigned\hspace{0.1cm} to\hspace{0.1cm} host\hspace{0.1cm} h$\\
$h_{\textbf{arch}}= architecture\hspace{0.1cm} of\hspace{0.1cm}host\hspace{0.1cm}h$\\
$Arch= Host\hspace{0.1cm}architectures\hspace{0.1cm}considered$
\caption{Constrained Optimization Problem}\label{alg:packer_solver}
\begin{algorithmic}[2]
%\scriptsize
\Procedure{Packer-Solver}{$Hosts$, $Tasks$}
\\
\Comment{find an appropriate host for tasks}
\For{$t$ $\in$ $Tasks$}
\State ($\exists$ $h$ $\in$ $Hosts$) such that,
%\State ($\forall$ $k$ $\in$ $RD$), $t_{\textbf{limit}}(k)$ $\in$ $RR$, 
\State $\forall$ $k$, $t_{\textbf{limit}}(k)$ $\leq$ ($h_{\textbf{limit}}(k)-[\sum_{\substack{\forall t^{'} \in h_{\textbf{tasks}}}}t^{'}_{\textbf{limit}}(k)] )$
\State $Constraints$($t$)
\EndFor
\EndProcedure
\\
\Procedure{Constraints}{$t$}
\State $\forall$ $l$,  $h_{\textbf{arch}}$ $\in$ $Arch$,
\State $t_{\textbf{norm}}(l) =NormalizeScore(t_{\textbf{sensitivity}}(l), h_{ \textbf{arch}})$,
\State ($\sum_{\forall t \in h_{\textbf{tasks}}$}}($t_{\textbf{norm}}(l)$)) $\leq$ $1$
\EndProcedure
\\
\Procedure{NormalizeScore}{$t_{\textbf{sensitivity}}(l)$, $h_{\textbf{arch}}$}
\State \small $Equations ~\ref{CPU sensitivity normalization}, ~\ref{Memory Bandwidth sensitivity normalization} \hspace{0.1cm} \& ~\ref{Network Bandwidth sensitivity normalization}\hspace{0.1cm}for\hspace{0.1cm}normalization\hspace{0.1cm}based\hspace{0.1cm}on\hspace{0.1cm}h_{arch}$\\
\Return $t_{\textbf{norm}}(l)$
\EndProcedure

\end{algorithmic}
}
\end{algorithm}



==> RelateWorkComparison.tex <==
\begin{equation}\label{Memory Bandwidth sensitivity normalization}
\resizebox{0.85\hsize}{!}{%
$MEMBW Sens_{Arch1} = \frac{MEMBW Sens_{Arch2} \times \frac{MEMBW_{Arch2}}{Cores_{Arch2}}}
{\frac{MEMBW_{Arch1}}{Cores_{Arch1}}}$%
}
\end{equation}

\begin{equation}\label{Network Bandwidth sensitivity normalization}
\resizebox{0.85\hsize}{!}{%

$NETBW Sens_{Arch1} = \frac{NETBW Sens_{Arch2} \times \frac{NETBW_{Arch2}}{Cores_{Arch2}}}
{\frac{NETBW_{Arch1}}{Cores_{Arch1}}}$%
}
\end{equation}




\begin{table*}
\begin{tabularx}{\textwidth}{|| X | X | X | X | X | X ||} 

 \hline
 
\textbf{Related Work }& \textbf{Workloads/QoS} & \textbf{Architectural Heterogeneity} &\textbf{Overheads} & \textbf{Scale} & \textbf{Drawbacks} \\ [0.5ex] 
 \hline\hline
\textcolor{blue}{Bubble-Up\cite{Bubble-Up}} & One Latency-sensitive and One Batch/ Assumes availability of well defined QoS metrics& Normalized sensitivity scores? Architecture specific scores? & Offline sensitivity analysis required to store bubble graph and score  & At scale difficult\textit{O(N)}(applications pressure on memory and application sufferance at different levels of pressure (sensitivity curve)) & Pairwise sensitivity data required, haven't considered modern workloads and architectures\\  
\hline
\textcolor{blue}{PerfIso\cite{PerfIso}} & One Latency-critical with One batch & No & Keep reserved set of cores for LC& Scalable & Reserving set of isolate cores causes internal fragmentation\\  
\hline
\textcolor{blue}{Autopilot\cite{Autopilot}} &Latency-critical and Batch  & No. &Machine Learning based method &  & \\  
\hline
\textcolor{blue}{Azure/Resource-central\cite{Azure}\cite{ResourceCentral}} & Delay sensitive vs delay-insensitive  &  & Offline VM characterization and Machine Learning& Uses Microsoft's internal TLC for ML, offline characteristics of VMs running needed & Caches prediction results, models, and features on client side \\  
\hline
\textcolor{blue}{PARTIES\cite{PARTIES}} & One or more Latency-sensitive and One or more Batch (well defined QoS)& No & Fungability of resources need to be know  & QoS requirement &Finite state machine not exploring other possibilities \\[1ex] \hline
\end{tabularx}
\caption{\textcolor{blue}{Related work comparison (Compare against Bubble-Up, PARTIES, Autopilot public clouds, AzurePublicDataset paper)}}
\label{RelatedWorkComparison}
\end{table*}

\iffalse
\begin{center}
\begin{table}[t]
\resizebox{2\columnwidth}{!}{ \begin{tabular}{||c | c | c | c | c |c ||} 

 \hline
 
\textbf{Related Work }& \textbf{Workloads} & \textbf{Architectural Heterogeneity} &\textbf{Overheads} & \textbf{Scale} & \textbf{Drawbacks} \\ [0.5ex] 
 \hline\hline
Bubble-Up\cite{Bubble-Up} &  &  & &  & \\  
\hline
Autopilot\cite{Autopilot} &  &  & &  & \\  
\hline
Azure/Resource-central\cite{Azure}\cite{ResourceCentral} &  &  & &  & \\  
\hline
PARTIES\cite{PARTIES} &  &  & &  & \\[1ex] \hline

\end{tabular}}
\caption{\textcolor{blue}{Related work comparison (Compare against Bubble-Up, PARTIES, Autopilot public clouds, AzurePublicDataset paper)}}
\label{RelatedWorkComparison}
\end{table}
\end{center}
\fi

\iffalse
\begin{table}[!h]
\resizebox{\columnwidth}{!}{\begin{tabular}{||l|l|l|l|l|l|l|||}
\hline
\textbf{Services} &  \textbf{Haswell10} & \textbf{Haswell12} & \textbf{Skylake14} & \textbf{Skylake16} & \textbf{Broadwell18} & \textbf{Broadwell20}\\
\hline
\hline
\multirow{1}{*}{Log1}&0.83&0.75&1.04&0.53&1.34&0.68\\
\hline
\multirow{1}{*}{KeyVal1}&0.77&0.7&0.97&0.5&1.25&0.63\\
\hline
\multirow{1}{*}{NN1}&0.77&0.7&0.97&0.5&1.26&0.63\\
  \hline
\multirow{1}{*}{KeyVal2}&0.75&0.75&1.00&0.45&1.13&0.64\\
  \hline
\multirow{1}{*}{KeyVal3}&0.99&0.9&1.24&0.64&1.61&0.81\\
\hline
\multirow{1}{*}{Rank2}&1.13&1.03&1.42&0.73&1.84&0.93\\
\hline
\hline
\end{tabular}}
\caption{CPU Sensitivity Scores}\label{CPU service sensitivity}
\end{table}

\begin{table}[!h]
\resizebox{\columnwidth}{!}{\begin{tabular}{||l|l|l|l|l|l|l|||}
\hline
\textbf{Services} &  \textbf{Haswell10} & \textbf{Haswell12} & \textbf{Skylake14} & \textbf{Skylake16} & \textbf{Broadwell18} & \textbf{Broadwell20}\\
\hline
\hline
\multirow{1}{*}{Log1}&0.92&0.58&0.69&0.68&1.11&0.60\\
\hline
\multirow{1}{*}{KeyVal1}&0.63&0.4&0.47&0.47&0.76&0.41\\
\hline
\multirow{1}{*}{NN1}&0.81&0.51&0.61&0.6&0.98&0.53\\
  \hline
\multirow{1}{*}{KeyVal2}&0.92&0.58&0.92&0.41&1.65&0.45\\
  \hline
\multirow{1}{*}{KeyVal3}&1.15&0.73&0.86&0.86&1.39&0.76\\
\hline
\multirow{1}{*}{Rank2}&1.31&0.83&0.98&0.97&1.58&0.86\\
\hline
\hline
\end{tabular}}
\caption{Memory bandwidth Sensitivity Scores}\label{MemBw service sensitivity}
\end{table}

\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{\begin{tabular}{||l|l|l|l|l|l|l|||}
\hline
\textbf{Services} &  \textbf{Haswell10} & \textbf{Haswell12} & \textbf{Skylake14} & \textbf{Skylake16} & \textbf{Broadwell18} & \textbf{Broadwell20}\\
\hline
\hline
\multirow{1}{*}{Log1}&1.32 &1.32&0.19&0.83&0.17&0.6\\
\hline
\multirow{1}{*}{KeyVal1}&1.32 &1.32&0.19&0.83&0.17&0.61\\
\hline
\multirow{1}{*}{NN1}&0.8 &0.8&0.12&0.50&0.10&0.36\\
  \hline
\multirow{1}{*}{KeyVal2}&1.12 &1.12&0.16&0.7&0.14&0.51\\
  \hline
\multirow{1}{*}{KeyVal3}&1.98 &1.98&0.27&1.24&0.25&0.9\\
\hline
\multirow{1}{*}{Rank2}&1.98 &1.98&0.27&1.24&0.25&0.96\\
\hline
\hline
\end{tabular}}
\caption{Network bandwidth Sensitivity Scores}\label{NetBw service sensitivity}
\end{table}

\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
\begin{table}[htbp]
\resizebox{\columnwidth}{!}{\begin{tabular}{||l|l|l|l|l|l|l|||}
\hline
\textbf{Services} &  \textbf{Haswell T1} & \textbf{Haswell T6} & \textbf{Skylake T1} & \textbf{Skylake T6} & \textbf{Broadwell T1} & \textbf{Broadwell T6}\\
\hline
\hline
\multirow{3}{*}{adlogger}&CPU=0.83&CPU=0.75&CPU=1.04&CPU=0.53&CPU=1.34&CPU=0.68\\
    &MemBW=0.92&MemBW=0.58&MemBW=0.69&MemBW=0.68&MemBW=1.11&MemBW=0.60\\
    &NetBW= &NetBW=&NetBW=&NetBW=&NetBW=&NetBW=\\
\hline
\multirow{3}{*}{asx\_reader\_cold}&CPU=0.77&CPU=0.7&CPU=0.97&CPU=0.5&CPU=1.25&CPU=0.63\\
    &MemBW=0.63&MemBW=0.4&MemBW=0.47&MemBW=0.47&MemBW=0.76&MemBW=0.41\\
    &NetBW= &NetBW=&NetBW=&NetBW=&NetBW=&NetBW=\\
\hline
\multirow{3}{*}{embedding\_service}&CPU=0.77&CPU=0.7&CPU=0.97&CPU=0.5&CPU=1.26&CPU=0.63\\
    &MemBW=0.81&MemBW=0.51&MemBW=0.61&MemBW=0.6&MemBW=0.98&MemBW=0.53\\
    &NetBW= &NetBW=&NetBW=&NetBW=&NetBW=&NetBW=\\
\hline
\multirow{3}{*}{up2x\_read}&CPU=0.75&CPU=0.75&CPU=1.00&CPU=0.45&CPU=1.13&CPU=0.64\\
    &MemBW=0.92&MemBW=0.58&MemBW=0.92&MemBW=0.41&MemBW=1.65&MemBW=0.45\\
    &NetBW= &NetBW=&NetBW=&NetBW=0.7&NetBW=&NetBW=\\
\hline
\multirow{3}{*}{asx\_reader\_hot}&CPU=0.99&CPU=0.9&CPU=1.24&CPU=0.64&CPU=1.61&CPU=0.81\\
    &MemBW=1.15&MemBW=0.73&MemBW=0.86&MemBW=0.86&MemBW=1.39&MemBW=0.76\\
    &NetBW= &NetBW=&NetBW=&NetBW=&NetBW=&NetBW=\\
\hline
\multirow{3}{*}{adfinder}&CPU=1.13&CPU=1.03&CPU=1.42&CPU=0.73&CPU=1.84&CPU=0.93\\
    &MemBW=1.31&MemBW=0.83&MemBW=0.98&MemBW=0.97&MemBW=1.58&MemBW=0.86\\
    &NetBW= &NetBW=&NetBW=&NetBW=&NetBW=&NetBW=\\
\hline
\hline
\end{tabular}}
\caption{Sensitivity scores}\label{service sensitivity}
\end{table}
\fi
%%%%%%%%%
\iffalse
\begin{center}
\begin{table}[h!]
\resizebox{\columnwidth}{!}{ \begin{tabular}{||c | c | c | c | c ||} 
 \hline
 Architectures & Cores & Memory (in GB) & Memory Bandwidth (in GBps) & Network Bandwidth (in Gbps) \\ [0.5ex] 
 \hline\hline
Haswell T1 & 48 & 32 & 75.6 & 5 \\ 
 \hline
Haswell T6 & 48 & 256 & 120 & 5 \\
 \hline
Skylake T1 & 36 & 64 & 76 & 25\\
 \hline
Skylake T6 & 80 & 256 & 170 & 12.5\\
 \hline
Broadwell T1 & 32 & 32 & 42 & 25\\ 
\hline
Broadwell T6 & 56 & 256 & 153 & 12.5\\ [1ex] 
\hline
\end{tabular}}
\caption{Comparison between different architectures}
\label{Architectures}
\end{table}
\end{center}
\fi
%%%%%%%
\iffalse
\begin{center}
\begin{table}[h!]
\resizebox{\columnwidth}{!}{ \begin{tabular}{||c | c | c | c | c ||} 
 \hline
 Architectures & mRCU & RCU & Memory Bandwidth/Cores (in GBps) & Network Bandwidth/Cores (in Gbps) \\ [0.5ex] 
 \hline\hline
Haswell T1 & 8 & 4.20 & 1.58 & 0.10 \\ 
 \hline
Haswell T6 & 24 & 4.62 & 2.50 & 0.10\\
 \hline
Skylake T1 & 13& 3.33 & 2.11 & 0.69\\
 \hline
Skylake T6 & 40 & 6.50 & 2.13 & 0.16\\
 \hline
Broadwell T1 & 11 & 2.58 & 1.31 & 0.78\\ 
\hline
Broadwell T6 & 30 & 5.10 & 2.41 & 0.22\\ [1ex] 
\hline
\end{tabular}}
\caption{Relative costs, RCU = Relative Compute Unit}
\label{Costs}
\end{table}
\end{center}
\fi

\iffalse
\begin{center}
\begin{table}[h!]
\resizebox{\columnwidth}{!}{ \begin{tabular}{||c ||c  ||} 
 \hline
 Service & Characterization \\ [0.5ex] 
 \hline\hline
Service A (Adlogger) & Web (Machine Learning) \\ 
 \hline
Service B (Asx\_reader\_cold) & In-Memory Key-Value Store (filters out inactive keys, loads full datasets, uses more memory less compute)\\
 \hline
Service C (embedding\_Service) & Nearest-Neighbor(NN) search \\
 \hline
Service D (up2x\_read) & Customized Key-Value store\\
 \hline
Service E (asx\_reader\_hot)&In-Memory Key-Value Store (filters out active keys, loads less datasets, uses more compute less memory)\\
\hline
Service F (adfinder) & Web\\ [1ex] 
\hline
\end{tabular}}
\caption{Service characterization}
\label{Service Characterization}
\end{table}
\end{center}
\fi
\iffalse
I don't think we need this table as we are not reveling any specific values.
\begin{center}
\begin{table}[h!]
\resizebox{\columnwidth}{!}{ \begin{tabular}{||c | c | c | c | c | c | c | c | c ||} 
 \hline
 Service & Core & Memory(in GB) & P90 Core & P90 Memory(in GB) & P95 Core  & P95 Memory(in GB) & P99 Core  & P99 Memory(in GB) \\ [0.5ex] 
 \hline\hline
Ads1 & 18 & 55 & 10 & 8.5&10&8.67&11&8.9 \\ 
 \hline
KeyVal1 & 24 & 248 & 1 & 208 &1 &208&1&209 \\
 \hline
KeyVal2 & 16 & 248 & 4 & 235&5&236&9&238\\ [1ex]
 \hline
 \hline
\end{tabular}}
\caption{Candidate services and percentile limits}
\label{Percentile limits}
\end{table}
\end{center}
\fi
\iffalse
\begin{figure}[h!] 
\begin{subfigure}{\columnwidth}
 \centering
\includegraphics[scale=0.30]{figure/3D_p95_T1.png} 
\caption{3D plot }
\label{TWADS T1 P95}
\end{subfigure}%
\newline
\begin{subfigure}{0.45\columnwidth}
  \centering
\includegraphics[scale=0.14]{figures/3D_cluster_p95_T1_3clusters.png} 
\caption{3 clusters}
\label{TWADS T1 P95 3 clusters}
\end{subfigure}\hfill%
%\hspace{0.05cm}
\begin{subfigure}{0.45\columnwidth}
  \centering
\includegraphics[scale=0.14]{figures/3D_cluster_p95_T1_4clusters.png} 
\caption{4 Clusters}
\label{TWADS T1 P95 4 clusters}
\end{subfigure}%
\caption{Percentile 95 resource utilization cluster plot (Jobs on Type I hosts)}
\end{figure} 
\fi
\textbf{\iffalse
\begin{figure}[h!] 
\begin{subfigure}{\columnwidth}
 \centering
\includegraphics[scale=0.30]{figures/3D_p90_T1.png} 
\caption{3D plot }
\label{TWADS T1 P90}
\end{subfigure}%
\newline
\begin{subfigure}{0.45\columnwidth}
  \centering
\includegraphics[scale=0.14]{figures/3D_cluster_p90_T1_3clusters.png} 
\caption{3 clusters}
\label{TWADS T1 P90 3 clusters}
\end{subfigure}\hfill%
%\hspace{0.05cm}
\begin{subfigure}{0.45\columnwidth}
  \centering
\includegraphics[scale=0.14]{figures/3D_cluster_p90_T1_4clusters.png} 
\caption{4 Clusters}
\label{TWADS T1 P90 4 clusters}
\end{subfigure}%
\caption{Percentile 90 resource utilization cluster plot (Jobs on Type I hosts)}
\end{figure} 
\fi
}
\iffalse
\begin{table}[htbp]
\resizebox{\columnwidth}{!}{\begin{tabular}{||l|l|l|l|l|l|l|||}
\hline
\textbf{Services} &  \textbf{Architecture 1} & \textbf{Architecture 2} & \textbf{Skylake14} & \textbf{Skylake16} & \textbf{Architecture 5} & \textbf{Broadwell20}\\
\hline
\hline
\multirow{3}{*}{Ads1}&CPU=0.83&CPU=0.75&CPU=1.04&CPU=0.53&CPU=1.34&CPU=0.68\\
    &MemBW=0.92&MemBW=0.58&MemBW=0.69&MemBW=0.68&MemBW=1.11&MemBW=0.60\\
    &NetBW=1.32 &NetBW=1.32&NetBW=0.19&NetBW=0.83&NetBW=0.17&NetBW=0.6\\
\hline
\multirow{3}{*}{KeyVal1}&CPU=0.77&CPU=0.7&CPU=0.97&CPU=0.5&CPU=1.25&CPU=0.63\\
    &MemBW=0.63&MemBW=0.4&MemBW=0.47&MemBW=0.47&MemBW=0.76&MemBW=0.41\\
    &NetBW=1.32 &NetBW=1.32&NetBW=0.19&NetBW=0.83&NetBW=0.17&NetBW=0.6\\
\hline
\multirow{3}{*}{NN1}&CPU=0.77&CPU=0.7&CPU=0.97&CPU=0.5&CPU=1.26&CPU=0.63\\
    &MemBW=0.81&MemBW=0.51&MemBW=0.61&MemBW=0.6&MemBW=0.98&MemBW=0.53\\
    &NetBW=0.8 &NetBW=0.8&NetBW=0.12&NetBW=0.50&NetBW=0.10&NetBW=0.36\\
\hline
\multirow{3}{*}{KeyVal2}&CPU=0.75&CPU=0.75&CPU=1.00&CPU=0.45&CPU=1.13&CPU=0.64\\
    &MemBW=0.92&MemBW=0.58&MemBW=0.92&MemBW=0.41&MemBW=1.65&MemBW=0.45\\
    &NetBW=1.12 &NetBW=1.12&NetBW=0.16&NetBW=0.7&NetBW=0.14&NetBW=0.51\\
\hline
\multirow{3}{*}{KeyVal3}&CPU=0.99&CPU=0.9&CPU=1.24&CPU=0.64&CPU=1.61&CPU=0.81\\
    &MemBW=1.15&MemBW=0.73&MemBW=0.86&MemBW=0.86&MemBW=1.39&MemBW=0.76\\
    &NetBW=1.98 &NetBW=1.98&NetBW=0.27&NetBW=1.24&NetBW=0.25&NetBW  =0.9\\
\hline
\multirow{3}{*}{Ads2}&CPU=1.13&CPU=1.03&CPU=1.42&CPU=0.73&CPU=1.84&CPU=0.93\\
    &MemBW=1.31&MemBW=0.83&MemBW=0.98&MemBW=0.97&MemBW=1.58&MemBW=0.86\\
    &NetBW=1.98 &NetBW=1.98&NetBW=0.27&NetBW=1.24&NetBW=0.25&NetBW  =0.9\\
\hline
\hline
\end{tabular}}
\caption{Sensitivity Scores}\label{service sensitivity}
\end{table}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{figure}[h!] 
\begin{subfigure}{\columnwidth}
  \centering
%\includegraphics[scale=0.30]{figures/3D_cluster_p99_T1_3clusters.png}
\includegraphics[scale=0.30]{figures/3D_cluster_new_p99_T1_twads_3clusters.png} 
\caption{3 clusters}
\label{TWADS T1 P99 3 clusters}
\end{subfigure}\hfill%
\vspace{0.5cm}
\iffalse
\begin{subfigure}{\columnwidth}
  \centering
\includegraphics[scale=0.25]{figures/cluster_info.png} 
\caption{Cluster information}
\label{cluster information}
\end{subfigure}%
\fi
\iffalse
\begin{subfigure}{\columnwidth}
  \centering
\includegraphics[scale=0.35]{figures/3D_cluster_p99_T1_4clusters.png} 
\caption{4 Clusters}
\label{TWADS T1 P99 4 clusters}
\end{subfigure}%
\fi
\caption{\textcolor{blue}{Resource utilization clustering based on measured p99 resource utilization among 3 dimensions (i) cpu, (ii) memory bandwidth and (iii) network bandwidth (on Type I hosts)}}
\end{figure} 
\fi
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{itemize}
    \item \textcolor{blue}{Background on Job scheduler (from Efficient, reliable cluster management at scale with Tupperware)}
        \begin{itemize}
            \item  \textcolor{blue}{cgroups used for basic isolation, resource partitioning done based on physical core counts and memory capacity.}
        \end{itemize}
    \item \textcolor{blue}{Packer-solver (Rebalancer) in details}
        \begin{itemize}
            \item \textcolor{blue}{Rebalancer packer-solver}
            \item \textcolor{blue}{Goals and Constraints}
            \item \textcolor{blue}{heterogeneity}
            \item \textcolor{blue}{at scale searches for local optima}
            \itme \textcolor{blue}{runs periodically}
        \end{itemize}    
    \item \textcolor{blue}{Taking care of peak resource utilization.}
     \begin{itemize}
         \item \textcolor{blue}{We take into account sensitivity scores which we describe as indirect inferred QoS metrics} 
         \item \textcolor{blue}{Since we calculate the percentile resource usage information based on 1 minute aggregated resource usage per task over a period of 7 days, we argue that we take care of resource fluctuations. } 
         
     \end{itemize}   
     \item \textcolor {blue} {Talk about candidate workloads in details}
        \item \textcolor{blue}{TCO aspect of bin packing host saving metrics}
\end{itemize}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{center}
\begin{table}[h!]
 \resizebox{\columnwidth}{!}{\begin{tabular}{||c | c ||}
 \hline
 Group & Host count \\ [0.5ex] 
 \hline\hline
group 1 & hosts $>=$ 100,000  \\ 
 \hline
group 2 & 100,000 $>$ hosts $>=$ 10,000 \\
 \hline
 group 3 & 10,000 $>$ hosts $>=$ 1000 \\
 \hline
 group 4 & 1000 $>$ hosts $>=$ 100 \\
 \hline
 group 5 & 100 $>$ hosts $>=$ 50 \\
 \hline
 group 6 & 50 $>$ hosts\\
 \hline
\end{tabular}}
\caption{\textcolor{blue}{Job groups based on hosts utilized}}
\label{Job groups}
\end{table}
\end{center}
\fi
%%%%%%%%%%%%%%%%%%

\iffalse
\begin{figure}[h!] 
\iffalse
\begin{subfigure}{\columnwidth}
 \centering
\includegraphics[scale=0.25]{figures/3D_p99_T6.png} 
\caption{3D plot }
\label{TWADS T6 P99}
\end{subfigure}%
\par\bigskip
\fi
\begin{subfigure}{\columnwidth}
  \centering
%\includegraphics[scale=0.30]{figures/3D_cluster_p99_T6_3clusters.png} 
\includegraphics[scale=0.30]{figures/3D_cluster_new_T6_tsp_3clusters.png} 

\caption{3 clusters}
\label{TWADS T6 P99 3 clusters}
\end{subfigure}\hfill%

\par\bigskip
\begin{subfigure}{\columnwidth}
  \centering
%\includegraphics[scale=0.30]{figures/3D_cluster_p99_T6_4clusters.png} 
%\caption{4 Clusters}
\label{TWADS T6 P99 4 clusters}
\end{subfigure}%
\caption{\textcolor{blue}{Resource utilization clustering based on measured p99 resource utilization among 3 dimensions (i) cpu, (ii) memory bandwidth and (iii) network bandwidth (on Type II hosts)}}
\end{figure} 
\fi
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\section{\textcolor{blue}{Background}}
\label{Background}
\textcolor{blue}{We use term tasks to refer to the schedulable entity with a configuration file that denotes it's resource limits. Resource isolation is ensured using cgroups for CPU and memory. Compute resource is allocated based on physical core counts and services have the option of using hyper-threaded contexts. A cluster manager is used for job deployment and resource management, applications are deployed on hosts in containers (cgroups). The cluster manager also monitors server health and is capable of moving tasks around in scenarios of server failures. A cluster manger agent runs on each server to orchestrate operation like creating, modifying or deleting containers. The cluster manager can manage resource utilization across datacenters and also, has capabilities of elastic compute.
}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%\vspace{-8.32cm}
We also observe from the resource utilization that there are only a few tasks that have high network bandwidth usage. Since we use the K-means clustering, for very closely placed tasks the clusterization can give rise to clusters with different characteristics. For example in figure ~\ref{clusters}, the clusters are not exactly based on low, medium and high resource utilization of all three dimensions. We observe that there are clusters with low compute, low memory and moderate network bandwidth utilization vs. low compute, high memory and moderate network bandwidth utilization vs. high compute, high memory and moderate network bandwidth utilization. This isn't orthogonal to our usage of the clustering information.\\
\fi
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%
%%%Commented out

\iffalse
\subsection{\textcolor{blue}{Similarity with Bubble-Up\cite{Bubble-Up}}}
\textcolor{blue}{Our method closely resembles the methodology for sensitivity analysis of Bubble-Up:}
\begin{itemize}

    \item \textcolor{blue}{Baseline is the utilization of the cluster when co-location is disallowed}
    \item \textcolor{blue}{In Bubble-Up the sensitivity curve is generated by stressing on the memory subsystem (shared cache, memory controller or memory bandwidth), this similar to the service-specific sensitivity scores we assign based on sensitivity analysis}
    \item \textcolor{blue}{We don’t use a reporter to keep track of how much the application itself stresses the memory subsystem}

\item\textcolor{blue}{ We rely on sensitivity scores of candidate workloads for bin packing}

\item \textcolor{blue}{Bubble-Up tested on 500 machines, with 17 workloads that have well defined QoS metrics and sensitivity is only taken into account for latency-sensitive workloads (QoS defined as 1/latency)}

\item \textcolor{blue}{Applications and resource needs might change, input load or source, hence, one-time characterization or sensitivity curves not advocated}

\item \textcolor{blue}{Limited to two applications, ours is not}
\end{itemize}
\textcolor{blue}{Differences:}
\begin{itemize}
    \item\textcolor{blue}{take into account actual resource usage limits (p99),} 
\item \textcolor{blue}{clusterization for workload characterization, }
\item \textcolor{blue}{normalization for heterogeneity,  and,}
\item \textcolor{blue}{tackle not only CPU fragmentation (cluster utilization) but also memory fragmentation and weighted host costs}

\item \textcolor{blue}{We advocate QoS that isn’t just latency oriented, and also, sensitivity assigned based on characterization using P99 resource limits and clustering
Multiple resource dimensions taken into account}
\end{itemize}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

